Temperature inhomogeneities cause the abundance discrepancy in H II regions

HII regions, ionized nebulae where massive star formation has taken place, exhibit a wealth of emission lines that are the fundamental basis for estimating the chemical composition of the Universe. For more than 80 years, a discrepancy of at least a factor of two between heavy-element abundances derived with collisional excited lines (CELs) and the weaker recombination lines (RLs) has thrown our absolute abundance determinations into doubt. Heavy elements regulate the cooling of the interstellar gas, being essential to the understanding of several phenomena such as nucleosynthesis, star formation and chemical evolution. In this work, we use the best available deep optical spectra of ionized nebulae to analyze the cause of this abundance discrepancy problem. We find for the first time general observational evidence in favor of the temperature inhomogeneities within the gas, quantified by t2. The temperature inhomogeneities inside H II regions are affecting only the gas of high ionization degree and producing the abundance discrepancy problem. This work implies that the metallicity determinations based on CELs must be revised, as they can be severely underestimated, especially in the regions of lower metallicity, such as the JWST high-z galaxies. We present methods to estimate these corrections, which will be critical for robust interpretations of the chemical composition of the Universe over cosmic time.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


